SynGen: A Syntactic Plug-and-play Module for Generative Aspect-based Sentiment Analysis

Aspect-based Sentiment Analysis (ABSA) is a sentiment analysis task at fine-grained level. Recently, generative frameworks have attracted increasing attention in ABSA due to their ability to unify subtasks and their continuity to upstream pre-training tasks. However, these generative models suffer from the neighboring dependency problem that induces neighboring words to get higher attention. In this paper, we propose SynGen, a plug-and-play syntactic information aware module. As a plug-in module, our SynGen can be easily applied to any generative framework backbones. The key insight of our module is to add syntactic inductive bias to attention assignment and thus direct attention to the correct target words. To the best of our knowledge, we are the first one to introduce syntactic information to generative ABSA frameworks. Our module design is based on two main principles: (1) maintaining the structural integrity of backbone PLMs and (2) disentangling the added syntactic information and original semantic information. Empirical results on four popular ABSA datasets demonstrate that SynGen enhanced model achieves a comparable performance to the state-of-the-art model with relaxed labeling specification and less training consumption.

==> 0_abstract_v0.tex <==
\begin{abstract}
Aspect-based Sentiment Analysis~(ABSA) is a sentiment analysis task at fine-grained level.
Recently, generative frameworks have attracted increasing attention in ABSA due to their ability to unify subtasks and their continuity to upstream pre-training tasks.
However, these generative models suffer from the neighboring dependency problem that induces neighboring words to get higher attention.
In this paper, we propose SynGen, a plug-and-play syntactic information aware module.
As a plug-in module, our SynGen can be easily applied to any generative framework backbones.
The key insight of our module is to add syntactic inductive bias to attention assignment and thus direct attention to the correct target words.
To the best of our knowledge, we are the first one to introduce syntactic information to generative ABSA frameworks.
Our module design is based on two main principles: (1) maintaining the \textbf{structural integrity} of backbone PLMs and (2) \textbf{decoupling} the added syntactic information and original semantic information.
Empirical results on four popular ABSA datasets demonstrate that SynGen enhanced model achieves a promising promotion compared to the original baseline.
\end{abstract}


% In this paper, we propose SynGen, a plug-and-play syntactic information aware module, which can be easily applied to any generative frameworks.
% By adding syntactic information to the generative ABSA models, our module effectively introduces syntactic inductive bias on attention assignment and thus solves the neighboring dependency problem.
% To the best of our knowledge, we are the first one to introduce syntactic information to generative ABSA frameworks.
% Moreover, our module maintains the structural integrity of backbone PLMs by inserting a parallel syntactic channel.
% To avoid the error accumulation from biased encoder output, we initialize the syntactic dependency tree based graph with pure POS embeddings.
% Empirical results demonstrate that the SynGen enhanced model achieves a promising promotion compared to the original baseline.

==> 1_introduction_v0.tex <==
\section{Introduction}
%第一段，ABSA简介
Aspect-based Sentiment Analysis~(ABSA)~\citep{14res_14lap} is a fine-grained sentiment analysis task.
A typical ABSA task includes three components: the aspects, sentiment polarities and opinions.
The goal of ABSA is to classify sentiment polarity around the aspect based on the corresponding opinion.
For example, in the sentence "\textit{The food is good but the service is bad}", the aspects are \textit{food} and \textit{service}, while the relevant opinions are \textit{good} and \textit{bad}, respectively.
According to the opinions, the sentiment polarity of the aspect \textit{food} is positive, and the sentiment polarity of \textit{service} is negative.
%拆成3句
%第一句Recently, generative frameworks are widely adopted in ABSA
%第二句 most生成式模型使用基于PLM的encoder-decoder的机构，把ABSA重定义/view/consider为文本生成任务
%第三局,他们的优势xxx
Recently, generative frameworks have been widely adopted for ABSA~\cite{unified_generative, SentiPrompt, generative1}.
Most of them are based on encoder-decoder structure Pre-trained Language Models~(PLMs) and view ABSA as a text generation task.
These generative frameworks achieve promising performance due to their ability of unifying ABSA subtasks and their continuity to upstream pre-training tasks.


%改成一个problem，重新描述一下
However, these generative frameworks suffer from neighboring dependency problem~\cite{neighboring, neighboring2} that induce neighboring words to get higher attention.
Such phenomenon was first observed by \citet{neighboring2} and \citet{neighboring} attributes it to the Masked Language Modeling~(MLM) pre-training task.
% the goal is to output (). @Taki
As illustrated in Figure 1, given the sentence "\textit{Food is always fresh and hot ready to eat!}", the target ABSA output should be (Food, hot, positive). 
But the baseline SPAN-BART~\citep{unified_generative}, which adopts BART~\citep{BART} as encoder and decoder, extracts a wrong triplet (Food, hot ready, positive) with a redundant word \textit{ready} in the opinion.
Since the words \textit{hot} and \textit{ready} are adjacents, the baseline SPAN-BART improperly treats them as a unit. 

\begin{figure}[t]
    \centering
    \includegraphics[width=\linewidth]{Figures/introduction_v4.pdf}
    \caption{The output for baseline SPAN-BART~\citep{unified_generative} and our SynGen under the same input sentence.%An illustration for the importance of structural information.
    The generative framework SPAN-BART extracts a redundant word \textit{ready} and our SynGen avoids this mistake by employing the syntactic information.}
\end{figure}

To address this issue, we propose SynGen, a plug-and-play syntactic information aware module.
% The key insight is to introduce syntactic inductive bias, thus avoid neighborhood dependency. @Taki
The key insight is to introduce syntactic inductive bias to attention assignment which will guide words to focus more on other related words.
%Since the syntactic information can provide an inductive bias on attention assignment, it will guide words to focus more on other related words.
In practice, we employ a syntactic dependency tree to model the syntactic information.
As shown in the lower portion of Figure 1, the adjacent words \textit{hot} and \textit{ready} are far apart from each other in the view of a syntactic dependency tree.
% Aware of this prior distance knowledge through xxx tree, the encoder can tell these words from a unit. @taki
Being aware of this prior distance knowledge through the dependency tree, the model can distinguish these words from a unit.

To properly adapt our module to the generative frameworks, we design the SynGen following two main principles: (1) maintaining the \textbf{structural integrity} of backbone PLMs and (2) \textbf{decoupling} the added syntactic information and original semantic information.

The goal of maintaining \textbf{structural integrity} is to narrow the gap with the upstream PLMs.
Since the PLM is sophisticated enough, any slightest unreasonable change will compromise the model performance.
For example, modeling syntactic information in the way of position embedding is intuitively impracticable.
% Because可以去掉，thus 后面改为 thus hurt the performance of capturing the semantic information. @Taki 
Simply adding the word embeddings with syntactic information embeddings will bring in non-pretrained input for the PLMs and thus hurt the performance of capturing the semantic information.
% by adding an independent syntactic channel -> by designing an independent channel to model syntactic information, which works in parallel with the PLM backbone @Taki
In this case, we implement our module by adding an independent syntactic channel which works in parallel with the PLM backbone.
We view the original encoder as a semantic channel and fuse this channel with a syntactic channel to get more comprehensive representations.
Moreover, we design a dynamic gate mechanism to point-wisely add the outputs from these two channels.

The goal of \textbf{decoupling} the added syntactic information and original semantic information is to avoid error accumulation.
Following previous studies~\cite{graph2, graph3, graph4, graph1}, we build a graph based on the syntactic dependency tree and use Graph Neural Networks~(GNN) to model the syntactic information.
% 改为: 过去的一些方法可能会用encoder的输出来初始化Graph节点。然而，用biased word representation 来建模 语法信息 可能会造成error accumulation. 因此，我们将这两个channel解耦开，通过仅仅使用POS信息来初始化这些节点。 @Taki
Considering the motivation of introducing syntactic information is to solve the neighboring dependency problem, the syntactic channel should exclude the influence of biased backbone output and provide independent results.
Hence, we don't initialize the graph nodes with the backbone encoder output since this biased word representation will lead to error accumulation.
Instead, we use a sequence of part-of-speech~(POS) tags corresponding to the original input words and purely initialize the graph nodes with POS embeddings.
% 这个细节可说可不说，不重要。@Taki
These POS embeddings are derived from a learnable POS embedding layer.
% practice -> perform, empirical results demonstrate that such decoupling strategy achieves a significant promotion. @Taki
We perform further study in Graph Nodes Initialization Section and empirical results demonstrate that such a decoupling strategy achieves a significant promotion.
Moreover, the parallel channel design and decoupling strategy make our SynGen a plug-and-play module, which means that it can be easily applied to any generative framework backbone.

In summary, our main contributions are as follows:

$\bullet$ We propose a plug-and-play module SynGen to introduce syntactic information to generative ABSA frameworks. 
To the best of our knowledge, we are the first one to solve neighboring dependency problems in generative frameworks by adding syntactic information.
% Specially, we employ the POS information only to initialize the graph nodes, regardless of the semantic information. 
% Such a decoupling strategy avoids adding noise to the model and allows for better performance in modeling structural information.

$\bullet$ We explore the importance of decoupling syntactic and semantic information in generative frameworks. 
Empirical results demonstrate that the decoupling strategy plays an important role in adding syntactic information.

$\bullet$ we implement experiments on popular ABSA datasets. 
The experimental results demonstrate that our module achieves a promising improvement compared to strong baselines.
% 这个感觉可以不说，是一种意料之内的事情，不是什么特别值得说的点 @Taki
Further studies show that our syntactic channel can effectively enhance the attention weights from aspects to target opinions.

==> 2_related_work.tex <==
\section{Related Work}
Within the broad-sense ABSA task, there are multiple subtasks that can be classified into two categories: single output subtasks and compound output subtasks.

The goal of single output subtasks is to extract one of the three components: aspect, opinion, and sentiment polarity.
Given an input sentence, Aspect Term Extraction~(AE)~\cite{AE1,AE2,AE3,AE4} and Opinion Term Extraction~(OE)~\cite{OE1,OE2,OE3} aim to extract the aspects and opinions, respectively.
Besides, given a sentence and a certain aspect, Aspect-level Sentiment Classification~(ALSC)~\cite{ALSC1,ALSC2,ALSC3,ALSC4,ALSC5} aims to classify sentiment polarity around the aspect and Aspect-oriented Opinion Extraction~(AOE)~\cite{D19,AOE2,AOE3} focuses on extracting corresponding opinions for the aspect.

Meanwhile, the output of compound output subtasks is a permutation of the three components.
Aspect Term Extraction and Sentiment Classification (AESC)~\cite{AESC1,AESC2} aims to extract aspects and classify their sentiment polarities jointly.
Models in this subtask are generally based on unified tagging schema and multi-task learning.
Pair Extraction is a subtask that matches the extracted aspects and opinions from the given sentence.
\citet{pair} introduces a span-based multi-task neural network to this subtask and overcomes the drawbacks of sequence tagging schema.
Triplet extraction~\cite{penga,triplet2,triplet1,pengb,triplet3} is the most current comprehensive subtask of ABSA aiming to extract aspects, sentiment polarities and opinions simultaneously. 

More recently, some studies attempt to manage all subtasks under one unified framework~\cite{unified1, unified2} and generative frameworks are widely adopted in this field due to their adaptability.
\citet{unified_generative} unifies all seven subtasks based on BART~\citep{BART} and employ point networks~\citep{pointer_network} to construct decoder.
\citet{SentiPrompt} adopts sentiment knowledge enhanced prompts to tune a generative unified ABSA framework.

Despite the success made by the generative frameworks in ABSA, these methods heavily rely on PLMs and rarely change model architecture.
\citet{seq2path} improves the beam search process that keeps multiple branches and excludes redundant branches by a pruning algorithm.
\citet{unified_generative} changes the generative search space from the entire vocabulary to the input token indexes.
\citet{SentiPrompt} concatenates prompt template before input sentence.
In general, these generative models either design the decoding strategy or reformulate the input format, but these changes can not solve the neighboring dependency problem.


% Non-generative ABSA models commonly use syntactic information as a type of supplementary knowledge, whereas it can be a valuable complement to semantic data.
% Among many studies, Graph Neural Networks~(GNN) is the most popular method for processing syntactic information, and these include Graph Convolutional Networks~(GCN) and Graph Attention Networks~(GAT) with syntactic dependency tree achieve outstanding performance~\cite{graph2, graph3, graph4, graph1}.
% Furthermore, there are also studies that process syntactic and semantic information separately~\citep{DualGraph, Exploring}, but they just concatenate distinct embedding directly, which is inefficient.
% Despite the fact that these models leverage structural information, they are incapable of unifying the ABSA subtasks under a single framework.
% Instead, our SynGen addresses the flaws of the above studies while also reserving their benefits.

==> 3_methedology_v0.tex <==
\section{Methodology}

\begin{figure*}[!h]
	\centering
	\includegraphics[width=\linewidth]{Figures/overview_v5.pdf}
	\caption{
	An overview of the SynGen enhanced model.
	The model contains a dual-channel encoder and a pointer network decoder.
	The dual-channel encoder models syntactic and semantic information in parallel and their outputs are fused by a dynamic gate mechanism.
	The decoder sequentially generates target predictions from the candidate indexes.
	}
	\label{framework}
% 	\vspace{-1 em}
\end{figure*}

\subsection{Task Formulation}
There are seven subtasks in ABSA, including single output subtasks AE, OE, ALSC, AOE and compound output subtasks AESC, Pair Extraction and Triplet Extraction.
The target object of these subtasks is a permutation of three elements~(aspect, sentiment polarity, opinion).
In this paper, we only implement experiments for compound output subtasks since they are more complex and more challenging.

Given an input sentence $X=[x_1, x_2, ..., x_n]$, the target output is a serious of predictions $Y=[p_1, p_2,$ $ ..., p_k]$, where $n$ and $k$ represent the number of tokens and predictions, respectively.
In each prediction, we use $a$ and $o$ to represent the aspect and opinion, use the superscripts $\cdot^s$ and $\cdot^e$ to indicate the start and end of the index, and use $s\in\{neutral, positive, negative\}$ to denote the sentiment polarity.

The prediction of compound output subtasks is as follows:

$\bullet$ Aspect Term Extraction and Sentiment Classification~(AESC): $p_i=[{a_i}^s, {a_i}^e, s_i]$,

$\bullet$ Pair Extraction~(Pair): $p_i=[{a_i}^s, {a_i}^e, {o_i}^s, {o_i}^e]$,

$\bullet$ Triplet Extraction~(Triplet): $p_i=[{a_i}^s, {a_i}^e,$ ${o_i}^s, {o_i}^e, s_i]$.


\subsection{Model Architecture}
In this paper, we choose SPAN-BART~\citep{unified_generative} as our backbone and enhance it with our plug-and-play module SynGen.
As shown in Figure 2, the enhanced model contains a dual-channel encoder and a pointer-network decoder, which are linked by a dynamic gate mechanism.
On the left side of the gate mechanism, the encoder is composed of a mainstream semantic information channel and a syntactic channel, through which the input sentence and its corresponding POS tags are modeled in parallel.
The outputs of these two channels are fused by the dynamic gate mechanism.
And on the right side of the gate mechanism, the decoder receives the fused encoder outputs and generates sequential predictions based on the requirement of the certain subtask
%\subsubsection{Dual-channel Encoder}



\subsubsection{Semantic Channel.} 
Following SPAN-BART, we employ BART Embed and BART Encoder~\citep{BART} in the semantic channel to model the input sentence $X$ into hidden states $H^{se}$.
We also employ $\langle s \rangle$ and $\langle /s \rangle$ as the special tokens to represent the beginning and ending, respectively.
Therefore, we can obtain sentence representation by:
\begin{align}
  \mathbf{E}^{se}& =\mathrm{BARTEmbed}(\mathrm{\langle s \rangle};X;\mathrm{\langle /s \rangle}) \nonumber\\
     & =[e^{se}_{\langle s \rangle}, e^{se}_1, e^{se}_2, ..., e^{se}_n, e^{se}_{\langle /s \rangle}], \\
  \mathbf{H}^{se} & =\mathrm{BARTEnocder}(\mathbf{E}^{se}),
\end{align}
where $\mathbf{E}^{se},\mathbf{H}^{se} \in \mathbb{R}^{(n+2) \times d}$, superscript $\cdot^{se}$ denote the semantic channel and $d$ is the hidden state dimension.

\subsubsection{Syntactic Channel.}
To model the syntactic information, we build a bidirectional graph
$\mathbf{G}$ based on the syntactic dependency tree.
The adjacent matrix $\mathbf{A} \in \mathbb{R}^{n \times n}$ of G  is defined as follows:
\begin{align}
  \mathbf{A}_{ij} = \begin{cases}
    1,&  \text{if}  \  x_i, x_j \  \text{connect in dependency tree}, \\
    0,&  \text{otherwise},
  \end{cases} 
\end{align}
where $x_i$ represents the \textit{i}-th word of the input sentence $X$.

After building the graph, we use a sequence of POS tags $P=[pos_1, pos_2, ..., pos_n]$ to initial the graph nodes.
Each POS tag $pos_i$ is derived from its corresponding word\footnote{We use the spaCy toolkit to obtain the dependency tree and part-of-speech~(POS) tags: \url{https://spacy.io/}.}.
Words that are tokenized into multiple tokens will correspond to the same number of POS tags.
% For each token in the input sentence $X$, there is a corresponding POS label in $P=[pos_1, pos_2, ..., pos_n]$ derived from its untokenized word. 
We use a learnable embedding layer $\mathrm{POSEmbed}$ to embed the POS labels as follows:
\begin{align}
  \mathbf{E}^{sy}=\mathrm{POSEmbed}(P)=[e^{sy}_1, e^{sy}_2, ..., e^{sy}_n],
\end{align}
where $\mathbf{E}^{sy} \in \mathbb{R}^{n \times d}$ and superscript $\cdot^{sy}$ represents the syntactic channel.
Then we initialize the graph nodes by the above POS embeddings as $h^0_i=e^{sy}_i$, where $i$ represents the $i$-th node in the graph.

%\mathbf{H}^0=[h^0_1, h^0_2, ..., h^0_n]=[e^{sy}_1, e^{sy}_2, ..., e^{sy}_n]
% where $\mathbf{A} \in \mathbb{R}^{n \times n}$ denotes the adjacent matrix of graph $\mathbf{G}$ and $h^l_n$ is the hidden states of the i-th node at the l-th layer.

%In particular, the graph nodes are solely initialized by POS embeddings without any semantic information.
After that, we employ the Graph Attention Networks~(GAT)~\citep{GAT} to update nodes embeddings:
\begin{align}
  %& \mathbf{H}^0 =[h^0_1, h^0_2, ..., h^0_n]=[e^{sy}_1, e^{sy}_2, ..., e^{sy}_n], \\
  & h^{l+1}_i = \sum_{j\in \mathcal{N}(i)}\alpha^l_{i,j}h^l_j W^l, \\
  & \alpha^l_{i,j} = \mathrm{softmax}_i(e^l_{i,j}), \\
  & e^l_{i,j} = \mathrm{LeakyReLU}([h_i W^l||h_j W^l] \overrightarrow{a}^T),
\end{align}
where $h^l_i \in \mathbb{R}^{1 \times d}$ is the hidden state of the $i$-th node in the $l$-th layer.
$W^l \in \mathbb{R}^{d \times d}$ and $\overrightarrow{a} \in \mathbb{R}^{1 \times 2d}$ denotes the learnable weight matrices.
In this study, the number of GAT layers $L$ is set to 2.
We let the syntactic channel output $\mathbf{H}^{sy}$ be equal to the last layer hidden states $\mathbf{H}^L$ of GAT.
Finally, we pad the output with zero embeddings to align with the special tokens $\langle s \rangle$ and $\langle /s \rangle$ in the semantic channel:
\begin{align}
   \mathbf{H}^{sy} = [\mathbf{0}; \mathbf{H}^{L}; \mathbf{0}].
\end{align}

\subsubsection{Dynamic Gate Mechanism} We design a gate mechanism to properly fuse the two channel outputs.
The gate mechanism can dynamically condition the syntactic channel weight based on the semantic channel output:
\begin{align}
    \mathbf{H}^{e} = \mathbf{H}^{se}+\sigma\{\mathrm{Linear}(\mathbf{H}^{se})\} \odot \mathbf{H}^{sy}.
\end{align}
$\mathrm{Linear}$ denotes a linear layer reducing the vector into one dimension and $\odot$ represents the Hadamard product. 
For the activate function $\sigma$, we use the sigmoid function. 

\subsubsection{Pointer Network Enhanced Decoder}
The decoder takes the fused encoder output $\mathbf{H}^{e}$ and previous decoder outputs $Y_{<t}=[y_1, y_2, ..., y_{t-1}]$ as input to predict the $t$-step output $y_t$.
We adopt point networks as our decoding strategy, which do not directly generate the extracted text but replace it with the word indexes.
Since $Y_{<t}$ is a sequence of indexes, an Index-to-Token module is applied to convert $Y_{<t}$ to the appropriate hidden states:
\begin{align}
  \hat{y}_t = \begin{cases}
    X_{y_t},&  \text{if}  \  y_t \  \text{is a pointer index},\\
    C_{y_t - n},&  \text{if} \  y_t \  \text{is a polarity index},
  \end{cases}
\end{align}
where $C=\{neutral, positive, negative\}$ is the sentiment polarity list.

After converting the previous decoder outputs $\hat{Y}_{<t}$, we use the BART decoder to get the $t$-step hidden state:
\begin{align}
  \mathbf{h}_t^d & = \mathrm{BARTDecoder}(\mathbf{H}^e; \hat{Y}_{<t}),
\end{align}
where the superscript $\cdot^d$ represents the decoder output and the subscript $t$ denotes the t-th step.

To predict the $y_t$ probability distribution, we construct the candidate hidden states $[\mathbf{\bar{H}^e};\mathbf{C}^d]$ which is a concatenation of composite encoder outputs $\mathbf{\bar{H}^e}$ and polarity embeddings $\mathbf{C}^d$. 
And then we make an inner product between candidate hidden states and decoder output $\mathbf{h}_t^d$:
\begin{align}
  & \mathbf{\hat{H}}^e = \mathrm{MLP}(\mathbf{H}^e), \\
  & \mathbf{\bar{H}}^e = \alpha \mathbf{\hat{H}}^e + (1-\alpha) \mathbf{E}^e, \\
  & \mathbf{C}^d = \mathrm{BARTEmbed}(C), \\
  & \mathrm{Pro}_t = \mathrm{softmax}([\mathbf{\bar{H}^e};\mathbf{C}^d]  \mathbf{h}_t^d),
\end{align}
where $\mathbf{E}^e,\mathbf{H}^e,\mathbf{\hat{H}}^e,\mathbf{\bar{H}}^e \in \mathbb{R}^{(n+2) \times d}$;  $\mathbf{C}^d \in \mathbb{R}^{3 \times d}$; $\alpha$ represents the proportionality coefficient and $\mathrm{Pro}_t \in \mathbb{R}^{(n+5)}$ is the predicted distribution of $y_t$ among candidate indices.

In the training phase, we use the negative log-likelihood as the loss function and adopt the teacher forcing method to optimize our model.
Moreover, in the inference phase, we use the beam search to generate the prediction result.

==> 4_experiments_v0.tex <==
\section{Experiments}
%主实验表格放在method里了



\subsection{Datasets}
We evaluate our method on four popular ABSA datasets, including Rest14, Laptop14, Rest15 and Rest16.
These original datasets are proposed by the SemEval Challenges~\cite{14res_14lap, 15res, 16res}.
To obtain high quality triplets, we adopt two relabeled version $D_a$ and $D_b$ provided by \citet{penga} and \citet{pengb}, respectively.

The first version $D_a$ distills the triplets based on \citet{D17} and \citet{D19}, and reformulates them into the form of $\langle a,o,s \rangle$.
The second version $D_b$ revises the $D_a$ and adds triplets with overlapping opinions which are missed in $D_a$.
Table 1 shows the statistics of the four datasets in two versions.

\begin{table}[h]
 \resizebox{\linewidth}{!}{
\begin{tabular}{ll|cc|cc|cc|cc}
\toprule
\multicolumn{2}{l|}{\multirow{2}{*}{\textbf{Dataset}}} & \multicolumn{2}{c|}{\textbf{14res}} & \multicolumn{2}{c|}{\textbf{14lap}} & \multicolumn{2}{c|}{\textbf{15res}} & \multicolumn{2}{c}{\textbf{16res}} \\
\multicolumn{2}{l|}{}                                  & \#s              & \#t              & \#s              & \#t              & \#s              & \#t              & \#s             & \#t              \\ \hline
\multirow{3}{*}{$\mathbf{D_a}$}    & \textbf{train}    & 1300             & 2145             & 920              & 1265             & 593              & 923              & 842             & 1289             \\
                                   & \textbf{dev}      & 323              & 524              & 228              & 337              & 148              & 238              & 210             & 316              \\
                                   & \textbf{test}     & 496              & 862              & 339              & 490              & 318              & 455              & 320             & 465              \\ \hline
\multirow{3}{*}{$\mathbf{D_b}$}    & \textbf{train}    & 1266             & 2338             & 906              & 1460             & 605              & 1013             & 857             & 1394             \\
                                   & \textbf{dev}      & 310              & 577              & 219              & 346              & 148              & 249              & 210             & 339              \\
                                   & \textbf{test}     & 492              & 994              & 328              & 543              & 148              & 485              & 326             & 514              \\ \bottomrule
\end{tabular}
 }
\centering
\caption{The statistics of four datasets in two versions. We use \#s and \#t to represent the number of sentences and triplets, respectively.}
\end{table}

% Please add the following required packages to your document preamble:
% \usepackage{multirow}
\begin{table*}[!t]
 \resizebox{\linewidth}{!}{
\begin{tabular}{lccc|ccc|ccc|ccc}
\toprule
\multirow{2}{*}{Model} & \multicolumn{3}{c|}{14res}                       & \multicolumn{3}{c|}{14lap}                       & \multicolumn{3}{c|}{15res}                       & \multicolumn{3}{c}{16res}                        \\ \cline{2-13} 
                      & AESC           & Pair           & Triplet        & AESC           & Pair           & Triplet        & AESC           & Pair           & Triplet        & AESC           & Pair           & Triplet        \\ \hline
CMLA+                   & 70.62          & 48.95          & 43.12          & 56.90          & 44.10          & 32.90          & 53.60          & 44.60          & 35.90          & 61.20          & 50.00          & 41.60          \\
RINANTE+                & 48.15          & 46.29          & 34.03          & 36.70          & 29.70          & 20.00          & 41.30          & 35.40          & 28.00          & 42.10          & 30.70          & 23.30          \\
Li-unified+             & 73.79          & 55.34          & 51.68          & 63.38          & 52.56          & 42.47          & 64.95          & 56.85          & 46.69          & 70.20          & 53.75          & 44.51          \\
Peng-two-stage         & 74.19          & 56.10          & 51.89          & 62.34          & 53.85          & 43.50          & 65.79          & 56.23          & 46.79          & 71.73          & 60.04          & 53.62          \\
JET-BERT               & --             & --             & 63.92          & --             & --             & 50.00          & --             & --             & 54.67          & --             & --             & 62.98          \\
Dual-MRC               & 76.57          & 74.93          & 70.32          & 64.59          & 63.37          & 55.58          & 65.14          & 64.97          & 57.21          & 70.84          & 75.71          & 67.40          \\
SPAN-BART              & 78.47          & 77.68          & 72.46          & 68.17          & 66.11          & 57.59          & 69.95          & 67.98          & 60.11          & 75.69          & \textbf{77.38} & 69.98          \\ \hline
Ours                   & \textbf{78.64} & \textbf{77.92} & \textbf{73.61} & \textbf{70.06} & \textbf{68.53} & \textbf{60.71} & \textbf{71.61} & \textbf{69.35} & \textbf{64.06} & \textbf{77.51} & 77.34          & \textbf{71.26} \\ \bottomrule
\end{tabular}
}
\centering
\caption{Comparison F1 scores for AESC, Pair and Triplet on the $D_a$ dataset. The best results are highlighted in bold. The suffix “+” denotes modified by \citet{penga} for being capable of AESC, Pair and Triplet.}
\end{table*}

% Please add the following required packages to your document preamble:
% \usepackage{multirow}
\begin{table*}[!t]
 \resizebox{\linewidth}{!}{
\begin{tabular}{lccc|ccc|ccc|ccc}
\toprule
\multirow{2}{*}{Model} & \multicolumn{3}{c|}{14res}                       & \multicolumn{3}{c|}{14lap}                       & \multicolumn{3}{c|}{15res}                       & \multicolumn{3}{c}{16res}                        \\ \cline{2-13} 
                      & P              & R              & F1             & P              & R              & F1             & P              & R              & F1             & P              & R              & F1             \\ \hline
CMLA+                   & 39.18          & 47.13          & 42.79          & 30.09          & 36.92          & 33.16          & 34.56          & 39.84          & 37.01          & 41.34          & 42.10          & 41.72          \\
RINANTE+                & 31.42          & 39.38          & 34.95          & 21.71          & 18.66          & 20.07          & 29.88          & 30.06          & 29.97          & 25.68          & 22.30          & 23.87          \\
Li-unified+             & 41.04          & 67.35          & 51.00          & 40.56          & 44.28          & 42.34          & 44.72          & 51.39          & 47.82          & 37.33          & 54.51          & 44.31          \\
Peng-two-stage         & 43.24          & 63.66          & 51.46          & 37.38          & 50.38          & 42.87          & 48.07          & 57.51          & 52.32          & 46.96          & 64.24          & 54.21          \\
JET-BERT               & 70.56          & 55.94          & 62.40          & 55.39          & 47.33          & 51.04          & 64.45          & 51.96          & 57.53          & 70.42          & 58.37          & 63.83          \\
SPAN-BART              & 65.52          & 64.99          & 65.25          & 61.41          & 56.19          & 58.69          & 59.14          & \textbf{59.38} & 59.26          & 66.60          & 68.68          & 67.62          \\ \hline
Ours                   & \textbf{71.40} & \textbf{72.33} & \textbf{71.86} & \textbf{65.82} & \textbf{57.86} & \textbf{61.49} & \textbf{65.53} & 59.18          & \textbf{62.19} & \textbf{73.21} & \textbf{69.65} & \textbf{71.39} \\ \bottomrule
\end{tabular}
}
\centering
\caption{Main results for Triplet on the $D_b$ dataset. The best results are highlighted in bold. The suffix “+” denotes modified by \citet{penga} for being capable of Triplet.}
% \vspace{-1.0 em}
\end{table*}

\subsection{Baselines}
To fairly evaluate the performance of the SynGen enhanced model, we choose the following baselines for three compound output ABSA subtasks:

% Please add the following required packages to your document preamble:
% \usepackage{multirow}

$\bullet$ \textbf{CMLA}~\citep{D17} proposes an end-to-end model to jointly extract aspect and opinion terms.

$\bullet$ \textbf{RINANTE}~\citep{RINANTE} uses automatically labeled data to improve the influence of the co-extraction model.

$\bullet$ \textbf{Li-unified}~\citep{Li-unified} tackles target-based sentiment analysis with a unified tagging scheme.

$\bullet$ \textbf{Peng-two-stage}~\citep{penga} uses a two-stage framework to firstly extract aspects, aspect-based sentiment and opinions, and then pair aspects with the corresponding opinions.

$\bullet$ \textbf{JET-BERT}~\citep{pengb} designs a position-aware tagging schema to jointly extract triplets.

$\bullet$ \textbf{Dual-MRC}~\citep{unified1} exploits a dual-MRC framework to jointly train a triplet extraction model with three objectives.

$\bullet$ \textbf{SPAN-BART}~\citep{unified_generative} proposes a unified generative framework to handle all ABSA subtasks under one framework.

For the first three baselines CMLA, RINANTE and Li-unified, the suffix “+” in Table 2 and Table 3 denotes that they are modified by \citet{penga} for being capable of AESC, Pair and Triplet.
Besides, we do not compare our model with Seq2Path~\citep{seq2path} since they apply augmentation to training data.



\subsection{Implement Details}
In this study, all experiments are implemented on a 24G RTX3090 GPU, taking about an hour to complete 200 epochs of training with a batch size of 48.
We employ the BART as the backbone and set the hidden dimensions to 768.
The GAT learning rate is set to 1e-5 and the other parts learning rate is set to 1e-4.

Following previous studies, we use precision~(P), recall~(R) and F1 scores as metrics.
Specifically, a predicted aspect or opinion is judged to be correct only if the predicted span exactly matches the start and end boundaries of the ground truth.

%----------------------------------------------------------
%消融实验
% Please add the following required packages to your document preamble:
% \usepackage{multirow}
\begin{table*}[!h]
 \resizebox{\linewidth}{!}{
\begin{tabular}{lccc|ccc|ccc|ccc}
\toprule
\multirow{2}{*}{Model} & \multicolumn{3}{c|}{14res}                       & \multicolumn{3}{c|}{14lap}                       & \multicolumn{3}{c|}{15res}                       & \multicolumn{3}{c}{16res}                        \\ \cline{2-13} 
                      & AESC           & Pair           & Tripelt        & AESC           & Pair           & Tripelt        & AESC           & Pair           & Tripelt        & AESC           & Pair           & Tripelt        \\ \hline
ours                   & 78.64          & \textbf{77.92} & \textbf{73.61} & \textbf{70.06} & \textbf{68.53} & \textbf{60.71} & \textbf{71.61} & \textbf{69.35} & \textbf{64.06} & \textbf{77.51} & \textbf{77.34} & \textbf{71.26} \\
\enspace w/o graph              & 77.54          & 76.40           & 71.92          & 70.05          & 67.85          & 60.29          & 70.50           & 68.92          & 62.86          & 73.04          & 75.84          & 69.13          \\
\enspace w/o gate               & 77.37          & 76.03          & 71.90           & 69.49          & 68.09          & 60.43          & 71.45          & 68.68          & 63.11          & 75.33          & 76.16          & 70.14          \\
\enspace w/o graph\&gate        & \textbf{78.72} & 77.09          & 73.36          & 68.21          & 65.84          & 58.17          & 65.80           & 63.44          & 57.44          & 74.84          & 75.06          & 68.82          \\ \bottomrule
\end{tabular}
}
\centering
\caption{Ablation study on $D_a$. The best results are highlighted in bold.}
\end{table*}

% Please add the following required packages to your document preamble:
% \usepackage{multirow}
\begin{table*}[!h]
 \resizebox{\linewidth}{!}{
\begin{tabular}{lccc|ccc|ccc|ccc}
\toprule
\multirow{2}{*}{Model} & \multicolumn{3}{c|}{14res}                      & \multicolumn{3}{c|}{14lap}                       & \multicolumn{3}{c|}{15res}                       & \multicolumn{3}{c}{16res}                        \\ \cline{2-13} 
                      & P             & R              & F1             & P              & R              & F1             & P              & R              & F1             & P              & R              & F1             \\ \hline
ours                   & \textbf{71.40} & \textbf{72.33} & \textbf{71.86} & \textbf{65.82} & 57.86          & 61.49          & \textbf{65.53} & \textbf{59.18} & \textbf{62.19} & 73.21          & \textbf{69.65} & \textbf{71.39} \\
\enspace w/o graph              & 70.73         & 71.73          & 71.23          & 64.57          & \textbf{58.96} & \textbf{61.64} & 63.84          & 57.53          & 60.52          & \textbf{73.32} & 67.90           & 70.51          \\
\enspace w/o gate               & 69.94         & 70.93          & 70.43          & 62.96          & 57.49          & 60.10           & 63.35          & 57.73          & 60.41          & 72.92          & 68.09          & 70.42          \\
\enspace w/o graph\&gate        & 69.02         & 71.73          & 70.35          & 63.19          & 57.12          & 60.00             & 62.36          & 57.73          & 59.96          & 71.28          & 67.12          & 69.14          \\ \bottomrule
\end{tabular}
}
\centering
\caption{Ablation study on $D_b$. The best results are highlighted in bold.}
%\vspace{-1.0 em}
\end{table*}

\subsection{Main Results}
Among all seven ABSA subtasks, we only select three compound output subtasks: AESC, Pair and Triplet in the experiment, since they are more complex and challenging.
Following previous works, we perform all three subtasks in dataset version $D_a$ and perform only Triplet Extraction in version $D_b$.
Table 2 and Table 3 give the main results of our experiments.

In version $D_a$, F1 values are employed to evaluate the model performance.
As shown in Table 2, SynGen enhanced model outperforms all baselines on 14res, 14lap and 15res, and achieves a comparable result to the strong baseline SPAN-BART on 16res.
Although the enhanced model is 0.04\% lower than SPAN-BART for Pair, it gets higher F1 scores by 1.82\% and 1.28\% for AESC and Triplet, respectively.
On average, the enhanced model obtains promising improvements of 1.39\% F1 for AESC, 1.00\% F1 for Pair and 2.38\% F1 for Triplet, which demonstrates the effectiveness of our SynGen.
Especially for Triplet, we get a 3.95\% F1 promotion on 15res, representing a convincing superiority of the method.

Moreover, to further evaluate the ability of our SynGen in Triplet Extraction, we conduct experiments in version $D_b$ and use precision~(P) and recall~(R) as additional metrics.
Table 3 shows the main results for Triplet Extraction in $D_b$.
We can observe that our SynGen enhanced model achieves better performance on all datasets under the precision and F1 metrics.
However, under recall metrics, the enhanced model is 0.2\% lower than SPAN-BART on $D_b$ 15res, but still has a 6.39\% and 2.93\% promotion in precision and F1 values, respectively.
On average, our method achieves significant improvements of 5.82\% precision, 2.45\% recall and 4.03\% F1.
In particular, our SynGen achieves a 6.61\% promotion on 14res at most in terms of F1 values.

In conclusion, the main experiment results demonstrate that our SynGen can largely improve the performance of ABSA generative frameworks by enhancing them with syntactic information.


\subsection{Extensive Experiments}

\subsubsection{Ablation Study}
To further evaluate the necessity of each part in SynGen, we implement an extensive ablation study in versions $D_a$ and $D_b$.
The experiment results are shown in Table 4 and Table 5.
Specifically, we remove the graph and gate mechanism in turn to verify the effectiveness of these two modules.
In the model w/o graph, we remove the dependency-tree-based graph in the syntactic channel and output the POS embeddings directly.
And in the model w/o gate, we simply add the outputs of two channels without the dynamic gate mechanism.
Finally, in the model w/o graph\&gate, we remove both the graph and gate mechanism and add the semantic channel output with POS embeddings.
To minimize the absence of syntactic information, we reserve the POS embeddings in all the ablated models.

As shown in Table 4 and Table 5, the intact SynGen achieves the best performance on most datasets, demonstrating that both the dependency-tree-based graph and gate mechanism are indispensable in our SynGen.
However, some ablated models slightly surpass the intact model, but the gap of F1 score is limited to 0.15\%.
Considering that we implement experiments on numerous datasets, this recession may be caused by the difference in datasets distribution.
Meanwhile, we observe that removing the dynamic gate mechanism leads to a larger drop than removing the graph.
Such a phenomenon strengthens the importance of the proper algorithm to integrate syntactic and semantic information.

\begin{figure}[h]
    \centering
    \includegraphics[width=0.96\linewidth]{Figures/node_initial_v3.pdf}
    \caption{Experiment results of graph node initialization. 
    % Comparison of three strategies to initialize the nodes in graph.
    The top right legends denote the three types of values used in different initialization strategies.
    Prefix Da\_ and Db\_ represent the dataset version of $D_a$ and $D_b$, respectively.}
    % \vspace{-1.0 em}
\end{figure}

\begin{figure*}[!t]
    \centering
    \includegraphics[width=\linewidth]{Figures/attn_weight_v1.pdf}
    \caption{The heat map of word attention weights.
    The highlighted cell represents the attention from aspect to the corresponding opinion, which is enhanced by our SynGen.}
    % \vspace{1.0 em}
\end{figure*}

\subsubsection{Graph Nodes Initialization}

In our proposed SynGen, we purely initialize the graph nodes with POS embeddings to decouple with the original semantic information.

To verify the effectiveness of this approach, we implement an additional experiment on Triplet Extraction subtask to compare the model performance with different nodes initial values.
Figure 3 gives the experiment results where "POS only", "Token only" and "Token\&POS" represent three types of values to be used in each initialization strategy.
As shown in Figure 3, initializing graph nodes with pure POS embeddings achieves the best performance among all eight datasets.
On average, the pure POS method outperforms the token-only method by 1.33\% and outperforms the token\&POS method by 1.19\%.
Intuitively, initializing with backbone encoder output will bring in biased word representations and thus leads to error accumulation.
Empirical results confirm this assumption and demonstrate that solely initializing the graph nodes with POS embeddings is the optimal solution in our SynGen. 





% We attribute this result to the degeneration of the syntactic channel when initializing graph nodes with token embeddings.
% In our dual-channel encoder, the semantic channel is based on a well-trained model BART while the syntactic channel is trained from scratch.

% Thus, adding token embeddings into the syntactic channel only yields low-quality semantic representations, which is equivalent to noise for high-quality semantic channel output.
% Moreover, with adding token embeddings, the syntactic channel may degenerate to a subprime semantic channel and lose the effect of syntax-aware enhancement.
% In contrast, initializing graph nodes with pure POS embeddings prevents the interference of semantic information and guarantees the purity of the syntactic channel.






\subsubsection{Attention Weight Study}
Intuitively, our SynGen can provide a syntactic inductive bias to the generative frameworks and thus address the neighboring dependency issue.
To evaluate this assumption, we implement experiments on two typical datasets, $\mathrm{Da\_14res}$ and $\mathrm{Db\_14res}$, and analyze the attention weight gap between SynGen enhanced model and the baseline model.
To fully evaluate the magnitude of attention weight gaps, we evaluate from three perspectives:

% The above experiments demonstrate that our SynGen can improve generative frameworks by introducing syntactic information, but the mechanism of this approach remains in doubt.
% One conjecture is that syntactic information provides an inductive bias that 
% syntactic information establishes connections between the aspects and their contexts and provides a new perspective on learning syntax-aware features.
% Therefore, our improvement may increase the attention weights from aspects to relative opinions and facilitate the generation of desired results.
% To verify our conjecture, we conduct experiments on two typical datasets, $\mathrm{Da\_14res}$ and $\mathrm{Db\_14res}$, and gather statistics on the attention weight gap between StrGen and the strong baseline SPAN-BART.
% Furthermore, to fully evaluate the magnitude of attention weight gaps, we evaluate from three perspectives:

$\bullet$ \textbf{Value} represents the absolute value gap of attention weights. 
For aspects or opinions with multiple tokens, we choose the average value of the span subtraction as the value gap.

$\bullet$ \textbf{Rank} denotes the changes in attention weight ranks. 
Same as the value gap, we use the mean value of aspect token ranks as a result.

$\bullet$ \textbf{Prop.} indicates the proportion difference between the two models.
Assume the sum of aspect attention weights is 1 and the attention weights from aspect to opinion in S  SynGen enhanced model and the baseline model are $A_{ours}$ and $A_{baseline}$, respectively, the prop. is calculated as follows: $prop. = (A_{ours}-A_{baseline})/A_{ours}$.


\begin{table}[h]
\begin{tabular}{lccc}
\toprule
\textbf{Dataset} & \textbf{Value} & \textbf{Rank} & \textbf{Prop.} \\ \hline
Da\_14res        & 0.00789        & 0.11065       & 0.36691        \\
Db\_14res        & 0.00155        & 0.28385       & 0.11654        \\ \bottomrule
\end{tabular}
\centering
\caption{An illustration on how SynGen contributes the attention weights from aspect to opinion.}
% \vspace{-1.0 em}
\end{table}

As shown in Table 6, with the enhancement of SynGen, the attention weights from aspect to opinion boost under all three perspectives.
Especially in terms of the proportion, the enhanced model achieves a relative promotion of 36.69\% in version $D_a$ and 11.65\% improvement in version $D_b$.
Moreover, Figure 4 gives an illustration of how SynGen contributes to the attention weights from aspects to opinions.
For the given sentence, "This place has the best sushi in the city.", subfigures (a), (b) and (c) shows the attention metrics of the SynGen enhanced model, baseline model and their subtraction.
We can observe that the attention from "\textbf{sushi}" to "\textbf{best}" is magnified by SynGen as highlighted in the red box.
Besides, inconsequential attention such as "\textbf{city}" to "\textbf{the}" is impaired.
In conclusion, the attention weight study demonstrates that our SynGEN successfully guides the attention from aspect to the corresponding opinion and thus solves the neighboring dependency problem.



==> 4_experiments_v1.tex <==



%----------------------------------------------------------------
%主实验表
% Please add the following required packages to your document preamble:
% \usepackage{multirow}

% Please add the following required packages to your document preamble:
% \usepackage{multirow}
\begin{table*}[]
\resizebox{1.6\columnwidth}{!}
{
\begin{tabular}{lccc|ccc|ccc|ccc}
\toprule
Model & \multicolumn{3}{c|}{14res}                       & \multicolumn{3}{c|}{14lap}                       & \multicolumn{3}{c|}{15res}                       & \multicolumn{3}{c}{16res}                        \\ \cline{2-13} 
                       & AESC           & Pair           & Triplet        & AESC           & Pair           & Triplet        & AESC           & Pair           & Triplet        & AESC           & Pair           & Triplet        \\ \hline
CMLA+                   & 70.62          & 48.95          & 43.12          & 56.90          & 44.10          & 32.90          & 53.60          & 44.60          & 35.90          & 61.20          & 50.00          & 41.60          \\
RINANTE+                & 48.15          & 46.29          & 34.03          & 36.70          & 29.70          & 20.00          & 41.30          & 35.40          & 28.00          & 42.10          & 30.70          & 23.30          \\
Li-unified+             & 73.79          & 55.34          & 51.68          & 63.38          & 52.56          & 42.47          & 64.95          & 56.85          & 46.69          & 70.20          & 53.75          & 44.51          \\
Peng-two-stage         & 74.19          & 56.10          & 51.89          & 62.34          & 53.85          & 43.50          & 65.79          & 56.23          & 46.79          & 71.73          & 60.04          & 53.62          \\
JET-BERT               & --             & --             & 63.92          & --             & --             & 50.00          & --             & --             & 54.67          & --             & --             & 62.98          \\
Dual-MRC               & 76.57          & 74.93          & 70.32          & 64.59          & 63.37          & 55.58          & 65.14          & 64.97          & 57.21          & 70.84          & 75.71          & 67.40          \\
SPAN-BART              & 78.47          & 77.68          & 72.46          & 68.17          & 66.11          & 57.59          & 69.95          & 67.98          & 60.11          & 75.69          & 77.38          & 69.98          \\
SyMux                  & 78.68          & \textbf{79.42} & \textbf{74.84} & \textbf{70.32} & 67.64          & 60.11          & 69.08          & \textbf{69.82} & 63.13          & \textbf{77.95} & \textbf{78.82} & \textbf{72.76} \\ \hline
Ours                   & \textbf{79.72} & 77.59          & 74.02          & 70.06          & \textbf{68.53} & \textbf{60.71} & \textbf{71.61} & 69.35          & \textbf{64.06} & 77.51          & 77.34          & 71.26          \\
\enspace w/o graph              & 77.54          & 76.40          & 71.92          & 70.05          & 67.85          & 60.29          & 70.50          & 68.92          & 62.86          & 73.04          & 75.84          & 69.13          \\
\enspace w/o gate               & 77.37          & 76.03          & 71.90          & 69.49          & 68.09          & 60.43          & 71.45          & 68.68          & 63.11          & 75.33          & 76.16          & 70.14          \\
\enspace w/o graph\&gate        & 78.72          & 77.09          & 73.36          & 68.21          & 65.84          & 58.17          & 65.80          & 63.44          & 57.44          & 74.84          & 75.06          & 68.82          \\ \bottomrule
\end{tabular}
}
\centering
\caption{Comparison F1 scores for AESC, Pair and Triplet. The best results are highlighted in bold. The suffix “+” denotes being modified by \citet{penga} for being capable of AESC, Pair and Triplet.}
\end{table*}
%----------------------------------------------------------------


\section{Experiments}

% \subsection{Datasets, Baselines and Implement Details}
\subsection{Experment Setting}
\textbf{Datasets.}
We evaluate our method on four popular ABSA datasets, including Rest14, Laptop14, Rest15 and Rest16.
These original datasets are proposed by the SemEval Challenges~\cite{14res_14lap, 15res, 16res}.
To obtain high quality triplets, we adopt a refined version provided by Haiyun Peng~\cite{penga} which distills the triplets based on two previous relabeld versions~\cite{D17, D19}.


\noindent \textbf{Baselines.}
To fairly evaluate the performance of the SynGen enhanced model, we choose the following baselines for three ABSA subtasks:
CMLA~\cite{D17}, RINANTE~\cite{RINANTE}, Li-unified~\cite{Li-unified}, Peng-two-stage~\cite{penga}, JET-BERT~\cite{pengb}, Dual-MRC~\cite{unified1}, SPAN-BART~\cite{unified_generative} and SynMux~\cite{SynMux}.


% \textbf{CMLA}~\cite{D17} proposes an end-to-end model to jointly extract aspect and opinion terms.
% \textbf{RINANTE}~\cite{RINANTE} uses automatically labeled data to improve the influence of the co-extraction model.
% $\bullet$ \textbf{Li-unified}~\cite{Li-unified} tackles target-based sentiment analysis with a unified tagging scheme.
% $\bullet$ \textbf{Peng-two-stage}~\cite{penga} uses a two-stage framework to firstly extract aspects, aspect-based sentiment and opinions, and then pair aspects with the corresponding opinions.
% $\bullet$ \textbf{JET-BERT}~\cite{pengb} designs a position-aware tagging schema to jointly extract triplets.
% $\bullet$ \textbf{Dual-MRC}~\cite{unified1} exploits a dual-MRC framework to jointly train a triplet extraction model with three objectives.
% $\bullet$ \textbf{SPAN-BART}~\cite{unified_generative} proposes a unified generative framework to handle all ABSA subtasks under one framework.
% $\bullet$ \textbf{SynMux}~\cite{unified_generative} proposes a unified generative framework to handle all ABSA subtasks under one framework.


\noindent \textbf{Implementation.}
In this study, all experiments are implemented on a 24G RTX3090 GPU, taking about an hour to complete 200 epochs of training with a batch size of 48.
We employ the BART as the backbone and set the hidden dimensions to 768.
The GAT learning rate is set to 1e-5 and the other parts learning rate is set to 1e-4.
Following previous studies, we use F1 scores as metrics and a predicted aspect or opinion is judged to be correct only if the predicted span exactly matches the start and end boundaries of the ground truth.



\subsection{Main Results}
As shown in Table 1, SynGen enhanced model outperforms the original baseline SPAN-BART for almost every task. 
Although it is 0.04\% lower than SPAN-BART for Pair, our enhanced model gets higher F1 scores by 1.82\% and 1.28\% for AESC and Triplet, respectively.

all baselines on 14res, 14lap and 15res, and achieves a comparable result to the strong baseline SPAN-BART on 16res.
Although the enhanced model is 0.04\% lower than SPAN-BART for Pair, it gets higher F1 scores by 1.82\% and 1.28\% for AESC and Triplet, respectively.
On average, the enhanced model obtains promising improvements of 1.39\% F1 for AESC, 1.00\% F1 for Pair and 2.38\% F1 for Triplet, which demonstrates the effectiveness of our SynGen.
Especially for Triplet, we get a 3.95\% F1 promotion on 15res, representing a convincing superiority of the method.

To further evaluate the necessity of each part in SynGen, we remove the graph and gate mechanism in turn to verify the effectiveness of these two modules.
In the model w/o graph, we remove the dependency-tree-based graph in the syntactic channel and output the POS embeddings directly.
And in the model w/o gate, we simply add the outputs of two channels without the dynamic gate mechanism.
Finally, in the model w/o graph\&gate, we remove both the graph and gate mechanism and add the semantic channel output with POS embeddings.
To minimize the absence of syntactic information, we reserve the POS embeddings in all the ablated models.
As shown in the Table 1, the ablation study demonstrates that both graph and gate mechanism are indispensable.


% \subsection{Extensive Experiments}

% \subsubsection{Ablation Study}
% To further evaluate the necessity of each part in SynGen, we implement an extensive ablation study in versions $D_a$ and $D_b$.
% The experiment results are shown in Table 4 and Table 5.
% Specifically, we remove the graph and gate mechanism in turn to verify the effectiveness of these two modules.
% In the model w/o graph, we remove the dependency-tree-based graph in the syntactic channel and output the POS embeddings directly.
% And in the model w/o gate, we simply add the outputs of two channels without the dynamic gate mechanism.
% Finally, in the model w/o graph\&gate, we remove both the graph and gate mechanism and add the semantic channel output with POS embeddings.
% To minimize the absence of syntactic information, we reserve the POS embeddings in all the ablated models.

% As shown in Table 4 and Table 5, the intact SynGen achieves the best performance on most datasets, demonstrating that both the dependency-tree-based graph and gate mechanism are indispensable in our SynGen.
% However, some ablated models slightly surpass the intact model, but the gap of F1 score is limited to 0.15\%.
% Considering that we implement experiments on numerous datasets, this recession may be caused by the difference in datasets distribution.
% Meanwhile, we observe that removing the dynamic gate mechanism leads to a larger drop than removing the graph.
% Such a phenomenon strengthens the importance of the proper algorithm to integrate syntactic and semantic information.

% \begin{figure}[h]
%     \centering
%     \includegraphics[width=0.96\linewidth]{Figures/node_initial_v3.pdf}
%     \caption{Experiment results of graph node initialization. 
%     % Comparison of three strategies to initialize the nodes in graph.
%     The top right legends denote the three types of values used in different initialization strategies.
%     Prefix Da\_ and Db\_ represent the dataset version of $D_a$ and $D_b$, respectively.}
%     % \vspace{-1.0 em}
% \end{figure}


% \subsubsection{Graph Nodes Initialization}

% In our proposed SynGen, we purely initialize the graph nodes with POS embeddings to decouple with the original semantic information.

% To verify the effectiveness of this approach, we implement an additional experiment on Triplet Extraction subtask to compare the model performance with different nodes initial values.
% Figure 3 gives the experiment results where "POS only", "Token only" and "Token\&POS" represent three types of values to be used in each initialization strategy.
% As shown in Figure 3, initializing graph nodes with pure POS embeddings achieves the best performance among all eight datasets.
% On average, the pure POS method outperforms the token-only method by 1.33\% and outperforms the token\&POS method by 1.19\%.
% Intuitively, initializing with backbone encoder output will bring in biased word representations and thus leads to error accumulation.
% Empirical results confirm this assumption and demonstrate that solely initializing the graph nodes with POS embeddings is the optimal solution in our SynGen. 








% \subsubsection{Attention Weight Study}
% Intuitively, our SynGen can provide a syntactic inductive bias to the generative frameworks and thus address the neighboring dependency issue.
% To evaluate this assumption, we implement experiments on two typical datasets, $\mathrm{Da\_14res}$ and $\mathrm{Db\_14res}$, and analyze the attention weight gap between SynGen enhanced model and the baseline model.
% To fully evaluate the magnitude of attention weight gaps, we evaluate from three perspectives:


% $\bullet$ \textbf{Value} represents the absolute value gap of attention weights. 
% For aspects or opinions with multiple tokens, we choose the average value of the span subtraction as the value gap.

% $\bullet$ \textbf{Rank} denotes the changes in attention weight ranks. 
% Same as the value gap, we use the mean value of aspect token ranks as a result.

% $\bullet$ \textbf{Prop.} indicates the proportion difference between the two models.
% Assume the sum of aspect attention weights is 1 and the attention weights from aspect to opinion in S  SynGen enhanced model and the baseline model are $A_{ours}$ and $A_{baseline}$, respectively, the prop. is calculated as follows: $prop. = (A_{ours}-A_{baseline})/A_{ours}$.


% \begin{table}[h]
% \begin{tabular}{lccc}
% \toprule
% \textbf{Dataset} & \textbf{Value} & \textbf{Rank} & \textbf{Prop.} \\ \hline
% Da\_14res        & 0.00789        & 0.11065       & 0.36691        \\
% Db\_14res        & 0.00155        & 0.28385       & 0.11654        \\ \bottomrule
% \end{tabular}
% \centering
% \caption{An illustration on how SynGen contributes the attention weights from aspect to opinion.}
% % \vspace{-1.0 em}
% \end{table}

% As shown in Table 6, with the enhancement of SynGen, the attention weights from aspect to opinion boost under all three perspectives.
% Especially in terms of the proportion, the enhanced model achieves a relative promotion of 36.69\% in version $D_a$ and 11.65\% improvement in version $D_b$.
% Moreover, Figure 4 gives an illustration of how SynGen contributes to the attention weights from aspects to opinions.
% For the given sentence, "This place has the best sushi in the city.", subfigures (a), (b) and (c) shows the attention metrics of the SynGen enhanced model, baseline model and their subtraction.
% We can observe that the attention from "\textbf{sushi}" to "\textbf{best}" is magnified by SynGen as highlighted in the red box.
% Besides, inconsequential attention such as "\textbf{city}" to "\textbf{the}" is impaired.
% In conclusion, the attention weight study demonstrates that our SynGEN successfully guides the attention from aspect to the corresponding opinion and thus solves the neighboring dependency problem.



==> 5_conclusion_v0.tex <==
\section{Conclusion}

In this paper, we propose SynGen, a plug-and-play syntactic information aware module.
By adding syntactic information to the generative ABSA models, our module effectively introduces syntactic inductive bias on attention assignment and thus solves the neighboring dependency problem.
To the best of our knowledge, we are the first one to introduce syntactic information to generative ABSA frameworks.
Moreover, our module maintains the structural integrity of backbone PLMs by inserting a parallel syntactic channel.
To avoid the error accumulation from biased encoder output, we initialize the syntactic dependency tree based graph with pure POS embeddings.
Empirical results demonstrate that the SynGen enhanced model achieves a promising promotion compared to the original baseline.
Initialization experiments confirms the necessity of our decoupling strategy.
Case study shows that our SynGen successfully directs the attention from aspect to target opinion.
In future work, we will explore applying our SynGen for other information extraction tasks, e.g. event detection and relation extraction. 

% We propose StrGen, a generative ABSA framework that captures the structured syntactic information for better representation of input context.
% In StrGen, we design the syntactic channel where the nodes of the syntactic graph are solely initialized by the POS information.
% Moreover, a point-wise gate mechanism is proposed to fuse the syntactic and semantic channels.
% Our StrGen performs better than other strong baselines on popular benchmarks. 
% Further study shows that such structured syntactic information can improve attention weights among aspect and opinion terms.
% In future work, we will explore combining the syntactic and semantic channels for lower time and memory costs.
